The role of slicing in test-driven development

Test-driven development (TDD) is a widely used agile practice. However, very little is known with certainty about TDD's underlying foundations, i.e., the way TDD works. In this paper, we propose a theoretical framework for TDD, with the following characteristics: 1) Each TDD cycle represents a vertical slice of a (probably also small) user story, 2) vertical slices are captured using contracts, implicit in the developers' minds, and 3) the code created during a TDD cycle is a sliced-based specification of a code oracle, using the contracts as slicing pre/post-conditions. We have checked the connections among TDD, contracts, and slices using a controlled experiment conducted in the industry.

==> snippets/div-alternative.tex <==
\begin{table*}[]
\centering
\caption{TDD session for the \lstinline{div()} function, using the wrong abstractions}
\label{tab:div-listing-alternative}
\begin{adjustbox}{totalheight=1\textheight}
\begin{tabular}{lll}
\multicolumn{1}{c}{\textit{Test}} & \multicolumn{1}{c}{\textit{Slice}} & \multicolumn{1}{c}{\textit{Code}} \\ \hline
% 1st row
\begin{minipage}{.45\linewidth}
\begin{lstlisting}
#define BOOST_TEST_MAIN
#include <boost/test/included/unit_test.hpp>

#include "div.hpp"
BOOST_AUTO_TEST_CASE (divide_1_by_1)
{
	const int DIVIDEND = 1;
	const int DIVISOR = 1;
	const int QUOTIENT = 1;
	const int REMAINDER = 0;
	int quotient;
	int remainder;
	
	div(DIVIDEND, DIVISOR, &quotient, &remainder);
	BOOST_CHECK_EQUAL(quotient, QUOTIENT);
	BOOST_CHECK_EQUAL(remainder, REMAINDER);
}
\end{lstlisting}
\end{minipage}
%
& \multicolumn{1}{l|}{} 
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.15\linewidth}
\ 
\end{minipage}
%
& \multicolumn{1}{l|}{}        
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.27\linewidth}
\begin{lstlisting}
void div(int x, int y, int* q, int* r) {
	*q = 1;
	*r = 0;
}
\end{lstlisting}
\end{minipage} \\ \hline
% 2nd row
\begin{minipage}{.45\linewidth}
\begin{lstlisting} 
//triangulation test
BOOST_AUTO_TEST_CASE (divide_2_by_2)
{
	const int DIVIDEND = 2;
	const int DIVISOR = 2;
	const int QUOTIENT = 1;
	const int REMAINDER = 0;
	int quotient;
	int remainder;
	
	div(DIVIDEND, DIVISOR, &quotient, &remainder);
	BOOST_CHECK_EQUAL(quotient, QUOTIENT);
	BOOST_CHECK_EQUAL(remainder, REMAINDER);
}
\end{lstlisting}
\end{minipage}
%
& \multicolumn{1}{l|}{} 
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.15\linewidth}
\ 
\end{minipage}
%
& \multicolumn{1}{l|}{}        
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.27\linewidth}
\begin{lstlisting}
void div(int x, int y, int* q, int* r) {
	*q = 1;
	*r = 0;
}
\end{lstlisting}
\end{minipage} \\ \hline 
% 3rd row
\begin{minipage}{.45\linewidth}
\begin{lstlisting}
BOOST_AUTO_TEST_CASE (divide_2_by_1)
{
	const int DIVIDEND = 2;
	const int DIVISOR = 1;
	const int QUOTIENT = 2;
	const int REMAINDER = 0;
	int quotient;
	int remainder;
	
	div(DIVIDEND, DIVISOR, &quotient, &remainder);
	BOOST_CHECK_EQUAL(quotient, QUOTIENT);
	BOOST_CHECK_EQUAL(remainder, REMAINDER);
}
\end{lstlisting}
\end{minipage}
%
& \multicolumn{1}{l|}{} 
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.15\linewidth}
\ 
\end{minipage}
%
& \multicolumn{1}{l|}{}        
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.27\linewidth}
\begin{lstlisting}
void div(int x, int y, int* q, int* r) {
	int t;
	
	if (x == y ) {
		*q = 1;
		*r = 0;
	} else {
		*q = 2;
		*r = 0;
	}
}
\end{lstlisting}
\end{minipage} \\ \hline
% 4th row
\begin{minipage}{.45\linewidth}
\begin{lstlisting} 
BOOST_AUTO_TEST_CASE (divide_4_by_1)
{
	const int DIVIDEND = 4;
	const int DIVISOR = 1;
	const int QUOTIENT = 4;
	const int REMAINDER = 0;
	int quotient;
	int remainder;
	
	div(DIVIDEND, DIVISOR, &quotient, &remainder);
	BOOST_CHECK_EQUAL(quotient, QUOTIENT);
	BOOST_CHECK_EQUAL(remainder, REMAINDER);
}
\end{lstlisting}
\end{minipage}
%
& \multicolumn{1}{l|}{} 
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.15\linewidth}
\ 
\end{minipage}
%
& \multicolumn{1}{l|}{}        
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.27\linewidth}
\begin{lstlisting}
void div(int x, int y, int* q, int* r) {
	int t;
	
	if (x == y ) {
		*q = 1;
		*r = 0;
	} else {
		*q = x;
		*r = 0;
	}
}
\end{lstlisting}
\end{minipage} \\ \hline 
% 5th row
\begin{minipage}{.45\linewidth}
\begin{lstlisting} 
Refactoring, followed by regression test
\end{lstlisting}
\end{minipage}
%
& \multicolumn{1}{l|}{} 
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.15\linewidth}
\ 
\end{minipage}
%
& \multicolumn{1}{l|}{}        
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.27\linewidth}
\begin{lstlisting}
void div(int x, int y, int* q, int* r) {
	int t;
	
	if (x == y )
		*q = 1;
	else
		*q = x;
		
	*r = 0;
}
\end{lstlisting}
\end{minipage} \\ \hline 
%
\end{tabular}
\end{adjustbox}
\end{table*}


==> snippets/swap-first-modified.tex <==
\begin{table*}[]
\centering
\caption{First TDD cycle for the \lstinline{swap()} function, modified. The header of the function has been defined in full, preventing subsequent changes in the tests}
\label{tab:swap-listing-1-modified}
\begin{tabular}{lll}
\multicolumn{1}{c}{\textit{Test}} & \multicolumn{1}{c}{\textit{Slice}} & \multicolumn{1}{c}{\textit{Code}} \\ \hline
\begin{minipage}{.45\linewidth}
\begin{lstlisting}
#define BOOST_TEST_MAIN
#include <boost/test/included/unit_test.hpp>

#include "swap.hpp"

BOOST_AUTO_TEST_CASE (x_gets_value_4)
{
	const int OLD_Y_VALUE = 4;
	int x;
	int y = OLD_Y_VALUE;

	swap(&x, &y);
	BOOST_CHECK_EQUAL(x, OLD_Y_VALUE);
}
\end{lstlisting}
\end{minipage}
%
& \multicolumn{1}{l|}{} 
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.12\linewidth}
$\{y = 4\}$\\
\sout{\texttt{t = *x;}}\\
$\{y = 4\}$\\
\texttt{*x = *y;}\\
$\{x = 4\}$\\
\sout{\texttt{*y = t;}}\\
$\{x = 4\}$\\
\end{minipage}
%
& \multicolumn{1}{l|}{}        
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.30\linewidth}
\begin{lstlisting}     
void swap(int* x, int* y) {
	*x = 4
}
\end{lstlisting}
\end{minipage}
\end{tabular}
\end{table*}

==> snippets/swap-first.tex <==
\begin{table*}[]
\centering
\caption{First TDD cycle for the \lstinline{swap()} function}
\label{tab:swap-listing-1}
\begin{tabular}{lll}
\multicolumn{1}{c}{\textit{Test}} & \multicolumn{1}{c}{\textit{Code}} \\ \hline
\begin{minipage}{.50\linewidth}
\begin{lstlisting}
#define BOOST_TEST_MAIN
#include <boost/test/included/unit_test.hpp>

#include "swap.hpp"

BOOST_AUTO_TEST_CASE (x_gets_value_4)
{
	const int NEW_VALUE = 4;
	int x;

	swap(&x);
	BOOST_CHECK_EQUAL(x, NEW_VALUE);
}
    \end{lstlisting}
\end{minipage}
%
& \multicolumn{1}{l|}{} 
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.35\linewidth}
\begin{lstlisting}
void swap(int* x) {
	*x = 4
}
\end{lstlisting}
\end{minipage}
%
\end{tabular}
\end{table*}

==> snippets/swap-full.tex <==
\begin{lstlisting}[caption={\lstinline{swap()} code},label={listing:swap-listing-full}]

void swap(int* x, int *y) {
	int t;
	
	t = *x;
	*x = *y;
	*y = t;
}
\end{lstlisting}


==> snippets/swap-second.tex <==
\begin{table*}[]
\centering
\caption{Second TDD cycle for the \lstinline{swap()} function}
\label{tab:swap-listing-2}
\begin{tabular}{lll}
\multicolumn{1}{c}{\textit{Test}} & \multicolumn{1}{c}{\textit{Slice}} & \multicolumn{1}{c}{\textit{Code}} \\ \hline
\begin{minipage}{.45\linewidth}
\begin{lstlisting}
#define BOOST_TEST_MAIN
#include <boost/test/included/unit_test.hpp>

#include "swap.hpp"

BOOST_AUTO_TEST_CASE (x_gets_value_4)
{
	const int OLD_Y_VALUE = 4;
	int x;
	int y = OLD_Y_VALUE;
  
	swap(&x, &y);
	BOOST_CHECK_EQUAL(x, OLD_Y_VALUE);
}

BOOST_AUTO_TEST_CASE (x_gets_value_5)
{
	const int OLD_Y_VALUE = 5;
	int x;
	int y = OLD_Y_VALUE;
  
	swap(&x, &y);
	BOOST_CHECK_EQUAL(x, OLD_Y_VALUE);
}
\end{lstlisting}
\end{minipage}
%
& \multicolumn{1}{l|}{} 
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.12\linewidth}
$\{y = Y\}$\\
\sout{\texttt{t = *x;}}\\
$\{y = Y\}$\\
\texttt{*x = *y;}\\
$\{x = Y\}$\\
\sout{\texttt{*y = t;}}\\
$\{x = Y\}$\\
\end{minipage}
%
& \multicolumn{1}{l|}{}        
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.30\linewidth}
\begin{lstlisting}
void swap(int* x, int *y) {

	*x = *y;
}
\end{lstlisting}
\end{minipage}
\end{tabular}
\end{table*}


==> snippets/swap-third.tex <==
\begin{table*}[]
\centering
\caption{Third TDD cycle for the \lstinline{swap()} function}
\label{tab:swap-listing-3}
\begin{tabular}{lll}
\multicolumn{1}{c}{\textit{Test}} & \multicolumn{1}{c}{\textit{Slice}} & \multicolumn{1}{c}{\textit{Code}} \\ \hline
\begin{minipage}{.45\linewidth}
\begin{lstlisting}
#define BOOST_TEST_MAIN
#include <boost/test/included/unit_test.hpp>

#include "swap.hpp"

BOOST_AUTO_TEST_CASE (x_gets_value_4)
{
	const int OLD_Y_VALUE = 4;
	int x;
	int y = OLD_Y_VALUE;
  
	swap(&x, &y);
	BOOST_CHECK_EQUAL(x, OLD_Y_VALUE);
}

BOOST_AUTO_TEST_CASE (x_gets_value_5)
{
	const int OLD_Y_VALUE = 5;
	int x;
	int y = OLD_Y_VALUE;
  
	swap(&x, &y);
	BOOST_CHECK_EQUAL(x, OLD_Y_VALUE);
}
    
BOOST_AUTO_TEST_CASE (y_gets_value_5) // No me gusta el nombre de este test
{
	const int OLD_X_VALUE = 5;
	const int OLD_Y_VALUE = 4;
	int x = OLD_X_VALUE;
	int y = OLD_Y_VALUE;
 
	swap(&x, &y);
	BOOST_CHECK_EQUAL(x, OLD_Y_VALUE);
	BOOST_CHECK_EQUAL(y, OLD_X_VALUE);
}
\end{lstlisting}
\end{minipage}
%
& \multicolumn{1}{l|}{} 
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.12\linewidth}
$\{y = Y \land X = x\}$\\
\texttt{t = *x;}\\
$\{y = Y \land X = t\}$\\
\texttt{*x = *y;}\\
$\{x = Y \land X = t\}$\\
\texttt{*y = t;}\\
$\{x = Y \land y = X\}$\\
\end{minipage}
%
& \multicolumn{1}{l|}{}        
%
\begin{minipage}{.01\linewidth}
\end{minipage}
\begin{minipage}{.30\linewidth}
\begin{lstlisting}
void swap(int* x, int *y) {
	int t;
	
	t = *x;
	*x = *y;
	*y = t;
}
\end{lstlisting}
\end{minipage}
\end{tabular}
\end{table*}

